Thermodynamics of surfactant-enriched binary-fluid systems

Surface-active agents (surfactants) release potential energy as they migrate from one of two adjacent fluids onto their fluid-fluid interface, a process that profoundly impacts the system's energy and entropy householding. The continuum thermodynamics underlying such a surfactant-enriched binary-fluid system has not yet been explored comprehensively. In this article, we present a mathematical description of such a system, in terms of balance laws, equations of state, and permissible constitutive relations and interface conditions, that satisfies the first and second law of thermodynamics. The interface conditions and permissible constitutive relations are revealed through a Coleman-Noll analysis. We characterize the system's equilibrium by defining equilibrium equivalences and study an example system. With our work, we aim to provide a systematically derived framework that combines and links various elements of existing literature, and that can serve as a thermodynamically consistent foundation for the (numerical) modeling of full surfactant-enriched binary-fluid systems.

==> Sections/Appendices/Graphical_abstract.tex <==
\section{Graphical Abstract}
\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{Figures/Graphic_abstract.pdf}
    \caption{For Table of Contents Only}
    \label{fig:graphicalabstract}
\end{figure}
